ClimART: A Benchmark Dataset for Emulating Atmospheric Radiative Transfer in Weather and Climate Models

Numerical simulations of Earth's weather and climate require substantial amounts of computation. This has led to a growing interest in replacing subroutines that explicitly compute physical processes with approximate machine learning (ML) methods that are fast at inference time. Within weather and climate models, atmospheric radiative transfer (RT) calculations are especially expensive. This has made them a popular target for neural network-based emulators. However, prior work is hard to compare due to the lack of a comprehensive dataset and standardized best practices for ML benchmarking. To fill this gap, we build a large dataset, ClimART, with more than \emph{10 million samples from present, pre-industrial, and future climate conditions}, based on the Canadian Earth System Model. ClimART poses several methodological challenges for the ML community, such as multiple out-of-distribution test sets, underlying domain physics, and a trade-off between accuracy and inference speed. We also present several novel baselines that indicate shortcomings of datasets and network architectures used in prior work. Download instructions, baselines, and code are available at: https://github.com/RolnickLab/climart

==> figures/latex/models_per_ood.tex <==
\begin{figure}
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{figures/figs/ood/bar_plots/model_FLUX_RMSE_OOD_bars.png}
      \caption{Test RMSE}
      \label{fig:ood_rmse}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{figures/figs/ood/bar_plots/model_FLUX_MBE_OOD_bars.png}
      \caption{Test MBE}
      \label{fig:ood_mbe}
    \end{subfigure}
          \caption{Test performance as a function of the OOD test set for our different baseline models. All models fail to generalize to historical and, in particular, future pristine-sky atmospheric conditions. Particularly the MLP has enormous troubles. }
  \label{fig:model_per_ood}
\end{figure}


==> figures/latex/models_per_year.tex <==
\begin{figure}
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{figures/figs/yearly/model_SW_FLUX_RMSE_per_year.png}
      \caption{Test RMSE}
      \label{fig:yearly_rmse}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=.95\linewidth]{figures/figs/yearly/model_SW_FLUX_MBE_per_year.png}
      \caption{Test MBE}
      \label{fig:yearly_mbe}
    \end{subfigure}
          \caption{Performance as a function of the test year for our different baseline models. Metrics are in $W/m^2$ and shown as the average over the vertical and over the up- and down-welling flux errors. 
          }
  \label{fig:model_per_year}
\end{figure}


==> tables/main_benchmark.tex <==
\begin{table*}[ht]
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.2}
\centering
\small
 \begin{tabular}{p{2cm}rrrrrrrrrrrrrr}
 \toprule
 & \multicolumn{3}{c}{\textbf{Pristine-sky}} & \multicolumn{3}{c}{\textbf{Clear-sky}} \\
\cmidrule(l){2-4} \cmidrule(l){5-8}
 
 \textbf{Model} & MAE & MBE & RMSE & MAE & MBE & RMSE \\ 
 \midrule

MLP	 & $0.3441 \pm 0.03$ & $-0.1599 \pm 0.10$ & $0.7165 \pm 0.03$ & & & \\ 
\rowcolor{rowbackground}
GCN	 & $0.5636 \pm 0.03$ & $0.0561 \pm 0.03$ & $1.2719 \pm 0.34$ & & & \\ 
GraphNet	 & $0.3094 \pm 0.03$ & $-0.0007 \pm 0.25$ & $0.6846 \pm 0.01$ & & & \\ 
\rowcolor{rowbackground}
CNN	 & $0.1784 \pm 0.03$ & $-0.1425 \pm 0.03$ & $0.3025 \pm 0.03$ & & & \\ 

\bottomrule
\end{tabular}
\caption{
\red{These are vertically averaged errors computed by (upwelling error + downwelling error)/2. I will add the more detailed statistics, split up by output variable, in a sec.. (Also adding errors for TOA/surface only.)}
We run several neural network architectures on \climart\ to emulate the shortwave down- and up-welling radiative fluxes. The reported metrics (in $W/m^2$) are averaged out over all test samples (years 2007-2014) and three random seeds.
We find that the CNN architecture provides the most skillful emulation in terms of MAE and RMSE, while the GraphNet provides the least biased errors.
}
\label{tab:ml_benchmark}
\end{table*}







==> tables/main_ml_benchmark_full.tex <==
\begin{table*}[ht]
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.2}
\centering
\small
 \begin{tabular}{p{2cm}rrrrrrrrrrrrrr}
 \toprule
 & \multicolumn{2}{c}{\textbf{Downwelling}} & \multicolumn{2}{c}{\textbf{Upwelling}}
 & \multicolumn{2}{c}{\textbf{Mean}}
  & \multicolumn{2}{c}{\textbf{Mean}}
  &   & \multicolumn{2}{c}{\textbf{Mean}} \\
\cmidrule(l){2-3} \cmidrule(l){4-5}
\cmidrule(l){6-7} \cmidrule(l){8-9}
 \textbf{Model} & RMSE & MBE & RMSE & MBE & RMSE & MBE & RMSE & MBE & RMSE & MBE \\ 
 \midrule

MLP	 & $0.822 \pm 0.04$ & $-0.056 \pm 0.14$ & $0.580 \pm 0.11$ & $-0.263 \pm 0.10$ & $0.701 \pm 0.04$ & $-0.160 \pm 0.10$ & $0.684 \pm 0.07$ & $-0.282 \pm 0.09$ & $0.573 \pm 0.06$ & $-0.208 \pm 0.10$ \\ 
\rowcolor{rowbackground}
GCN	 & $1.601 \pm 0.27$ & $-0.039 \pm 0.01$ & $0.817 \pm 0.33$ & $0.108 \pm 0.09$ & $1.209 \pm 0.25$ & $0.034 \pm 0.04$ & $1.260 \pm 0.70$ & $0.244 \pm 0.47$ & $0.815 \pm 0.12$ & $0.071 \pm 0.15$ \\ 
L-GCN	 & $1.299 \pm 0.29$ & $-0.254 \pm 0.09$ & $0.457 \pm 0.12$ & $-0.103 \pm 0.29$ & $0.878 \pm 0.09$ & $-0.179 \pm 0.10$ & $0.714 \pm 0.21$ & $-0.241 \pm 0.29$ & $0.440 \pm 0.09$ & $-0.048 \pm 0.21$ \\ 
\rowcolor{rowbackground}
GraphNet	 & $0.833 \pm 0.10$ & $-0.054 \pm 0.28$ & $0.463 \pm 0.17$ & $0.053 \pm 0.26$ & $0.648 \pm 0.04$ & $-0.001 \pm 0.25$ & $0.620 \pm 0.08$ & $0.017 \pm 0.29$ & $0.434 \pm 0.08$ & $-0.033 \pm 0.21$ \\ 
CNN	 & $0.351 \pm 0.02$ & $-0.142 \pm 0.01$ & $0.254 \pm 0.07$ & $-0.143 \pm 0.06$ & $0.303 \pm 0.03$ & $-0.142 \pm 0.03$ & $0.265 \pm 0.03$ & $-0.138 \pm 0.03$ & $0.284 \pm 0.05$ & $-0.177 \pm 0.04$ \\ 

\bottomrule
\end{tabular}
\caption{
We run several neural network architectures on \climart\ to emulate the shortwave down- and up-welling radiative fluxes. The reported metrics (in $W/m^2$) are averaged out over all test samples (years 2007-2014) and three random seeds.
We find that the CNN architecture provides the most skillful emulation in terms of MAE and RMSE, while the GraphNet provides the least biased errors.
}
\label{tab:ml_benchmark_full}
\end{table*}





==> tables/speed/ml_clearsky.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline 
    Model & CPU(512) & CPU(8192) & GPU(512) & GPU(8192)\tabularnewline
    \hline 
    $\boldsymbol{MLP}$ &0.2342 & 0.1961 & 0.0063 & \textbf{0.0024}
    \tabularnewline
    \hline 
    $\boldsymbol{CNN}$ &3.1477 & 3.4127 & 0.0344 & 0.0252
    \tabularnewline
    \hline
    $\boldsymbol{GCN}$ & 3.2921 & 4.1523 & 2.0575 & 2.3002 
    \tabularnewline
    \hline
    $\boldsymbol{GN}$ & 27.9643 & 28.5588 & 0.1726 & 0.1685
    \tabularnewline
    \hline
\end{tabular}
% \bigskip
\label{tab:ml_clearsky}
\medskip
\caption{\textbf{Clear-sky inference speed benchmarks} of ML models on different hardware configurations (in seconds). The number inside the parentheses represents the batch-size used for input. Clear-sky takes slightly longer than pristine-sky because of more input variables.}
\end{table}

==> tables/speed/rt_clearsky.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline 
RT Physics Model & CPU(2) & CPU(4) & CPU(16) & CPU(64)\tabularnewline
\hline 
$\boldsymbol{Shortwave}$ & 2.1740 & 2.1544 & 2.0252 & \textbf{1.9842}
\tabularnewline
\hline 
$\boldsymbol{Longwave}$ &2.6253
& 2.6103
& 2.5540
& \textbf{2.5325}
\tabularnewline
\hline
\end{tabular}
%\bigskip
\label{tab:RT_clearsky}
\medskip
\caption{\textbf{Clear-sky benchmarks} of physics-based model on different number of CPUs (given in parentheses) and where time is in seconds.}
\end{table}





==> tables/speed/rt_pristine.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline 
    RT Physics Model & CPU(2) & CPU(4) & CPU(16) & CPU(64)\tabularnewline
    \hline 
    $\boldsymbol{Shortwave}$ & 3.3919 & 3.3666 & 2.0988 & \textbf{1.9817}
    \tabularnewline
    \hline 
    $\boldsymbol{Longwave}$ &  3.4679 & 3.4578 & 2.5851 & \textbf{2.5019}
    \tabularnewline
    \hline
\end{tabular}
%\bigskip
\label{tab:RT-pristine}
\medskip
\caption{\textbf{Pristine-sky benchmarks} of physics-based model on different number of CPUs (given in parentheses) and where time is in seconds.}
\end{table}
